LabelAId: Just-in-time AI Interventions for Improving Human Labeling Quality and Domain Knowledge in Crowdsourcing Systems

Crowdsourcing platforms have transformed distributed problem-solving, yet quality control remains a persistent challenge. Traditional quality control measures, such as prescreening workers and refining instructions, often focus solely on optimizing economic output. This paper explores just-in-time AI interventions to enhance both labeling quality and domain-specific knowledge among crowdworkers. We introduce LabelAId, an advanced inference model combining Programmatic Weak Supervision (PWS) with FT-Transformers to infer label correctness based on user behavior and domain knowledge. Our technical evaluation shows that our LabelAId pipeline consistently outperforms state-of-the-art ML baselines, improving mistake inference accuracy by 36.7% with 50 downstream samples. We then implemented LabelAId into Project Sidewalk, an open-source crowdsourcing platform for urban accessibility. A between-subjects study with 34 participants demonstrates that LabelAId significantly enhances label precision without compromising efficiency while also increasing labeler confidence. We discuss LabelAId's success factors, limitations, and its generalizability to other crowdsourced science domains.

==> description.tex <==
Figure 1: An overview diagram of the LabelAId system, which contains one, a novel ML-based pipeline for detecting labeling mistakes, which is efficiently trained to infer label correctness based on user behavior and domain knowledge; and two, a real-time ML model and UI that tracks worker behavior and intervenes when an inferred mistake is occurring. LabelAId improves data quality and worker expertise by providing just-in-time feedback during crowdsource labeling.

Figure 2: Conceptual diagram of our LabelAId pipeline. Programmatic weak supervision, utilizing domain-specific knowledge and heuristics, is employed to annotate the raw data. Subsequently, the noisy labels generated from PWS are used to pre-train the inference model. Lastly, the inference model is fine-tuned using clean labels for the target downstream task.

Figure 3: This figure showcases the Project Sidewalk Labeling Interface. Part A displays the interface used for labeling. Part B lists the different types of labels that can be applied, such as "obstacle" or "clear path." Part C provides examples of severity ratings for surface problems, ranging from 1 to 5, with 5 being the most severe and indicating a surface impassable for wheelchair users.

Figure 4: Conceptual diagram of our FT-Transformer-based model architecture. First, the model transforms the hybrid features (e.g., two numerical and two categorical features) into unified embeddings. Subsequently, these embeddings are processed iteratively by the Transformer layer. The final output is based on the [CLS] token.

Figure 5: Graph comparing the performance of the LabelAId pipeline with traditional machine learning methods, with an increasing number of clean downstream labels. The x-axis, representing the number of labels, is on a logarithmic scale. An error bar of plus-minus sigma is shown for N = 3. The graph includes data points for each baseline model trained on 50, 100, 200, 500, and 1000 clean labels from the Seattle dataset. It also shows the performance of a pre-trained FT-Transformer fine-tuned on an equivalent number of clean downstream samples."

Figure 6: Selected typical inference false positives per label type, where the model incorrectly infers the label as correct when, in fact, the label is wrong. a, c, failed to differentiate between a curb ramp and a missing curb ramp. b, d, labeled a drainage swale near an intersection with no sidewalk. For e to j, labels has attributes for a correct label but there is ample space for a wheelchair user to pass. 

Figure 7: Selected typical inference false negatives per label type, where the model incorrectly infers the label as wrong when, in fact, the label is correct. a to c are labeled mid-block crossings, geospatial information for such footpaths/crossings are incomplete in OpenStreetMap. d is an exit for a public facility. For e to h, missing optional inputs. i and j are labels rated Missing Sidewalk with low severity.

Figure 8: This Figure illustrates the user flow diagram of LabelAId when implemented in Project Sidewalk. The process starts with a user placing a label using the Project Sidewalk interface. If LabelAId detects an error, a just-in-time intervention dialog appears. The user then has three options: keep the label, delete the label, or view common mistakes related to that label type. If the user chooses to view common mistakes, they can also navigate to a page showing correct examples.

Figure 9: This figure contains system screenshots of LabelAId as implemented in Project Sidewalk. Part A shows a pop-up dialog that appears when a user label error is detected, featuring a mistake title, rotating labeling tips, and three action buttons: "Yes, I am sure," "No, remove the label," and "View Common Mistakes." Parts B and C are screenshots of the Common Mistakes Page and Correct Examples Page, respectively. Both pages display the user's current label alongside 3-4 example labels for easy comparison.

Figure 10: This description presents data on user labeling precision. Part A features a raincloud plot, which combines a half violin plot and a box plot, to illustrate the difference in label precision between a control group and an intervention group. This is shown for overall precision and for five specific label types. Part B is a table that lists the mean, standard deviation, Mann-Whitney U value, and p-value for both groups. The table indicates that the intervention group had statistically significantly higher precision in the overall category, as well as for the "curb ramp" and "no curb ramp" label types.

Figure 11: Four screenshots demonstrating the features of Project Sidewalk's built-in labeling assistance. Screenshots A and B display example screens presented at the start of each route, showing different types of labels that rotate each time. Screenshots C and D show the 'How to Label' section, which participants can access at any point during the labeling process to receive guidance and instructions.

==> supplementart-materials.tex <==
There are three supplementary materials:

1- "orientation-slides.pdf" is a PDF containing the orientation presentation during user studies. 

2- "post-study-questionnaire.pdf" is a PDF that contains the pre-study questionnaire questions.

3- "post-study-questionnaire.pdf" is a PDF that contains the post-study questionnaire questions.
